Graphon Pooling in Graph Neural Networks

Graph neural networks (GNNs) have been used effectively in different applications involving the processing of signals on irregular structures modeled by graphs. Relying on the use of shift-invariant graph filters, GNNs extend the operation of convolution to graphs. However, the operations of pooling and sampling are still not clearly defined and the approaches proposed in the literature either modify the graph structure in a way that does not preserve its spectral properties, or require defining a policy for selecting which nodes to keep. In this work, we propose a new strategy for pooling and sampling on GNNs using graphons which preserves the spectral properties of the graph. To do so, we consider the graph layers in a GNN as elements of a sequence of graphs that converge to a graphon. In this way we have no ambiguity in the node labeling when mapping signals from one layer to the other and a spectral representation that is consistent throughout the layers. We evaluate this strategy in a synthetic and a real-world numerical experiment where we show that graphon pooling GNNs are less prone to overfitting and improve upon other pooling techniques, especially when the dimensionality reduction ratios between layers is large.

==> sec_graphon_nn.tex <==
%!TEX root = GPoolSGNNs_eusipco2020.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Graphon Neural Networks  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
 \centering\includegraphics[angle=-90,scale=0.47]{./figures/fig1T_v01.pdf}
 \caption{Different ways to obtain a graph from a underlying graphon.}
 \label{fig:graphfromgraphon}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A graphon is a symmetric measurable function $W:[0,1]^2\rightarrow\mathbb{R}$ with $0\leq W(x,y)\leq 1$. It was originally conceived as a graph limit for sequences of dense graphs whose number of nodes grows to infinity~\cite{lovasz2012large}. \blue{(More on graphons?)} Finite graphs can be obtained from graphons in multiple ways, among which are using sampling and piece-wise approximations (see Fig.~\ref{fig:graphfromgraphon}). In the first case, a graph $G=(V(G),E(G),\alpha)$ with node set $V(G)$, edge set $E(G)$ and weight function $\alpha:E(G)\rightarrow\mathbb{R}^{+}$ is obtained assigning to each node in $u\in V(G)$ the number $\varphi(u)\in [0,1]$, such that for any two nodes $u,v\in V(G)$ we have $\{u,v\}\in E(G)$ and $\alpha(\{u,v\})=W(\varphi(u),\varphi(v))$, where $\varphi: V(G)\rightarrow [0,1]$ is a mapping that defines partly \blue{(why parlty?)} the type of approximation that is considered to generate the graphs. In the second case a set of $\vert V(G)\vert-1$ points is selected in $[0,1]$ using $\varphi$ and for any two nodes $u,v\in V(G)$ we have that $\{u,v\}\in E(G)$ and
%%%%%%%%%%%%%%%%
\begin{equation} \label{eqn:integration}
\alpha(\{u,v\})=\frac{1}{\left\vert \varphi(u)-\varphi(v)\right\vert^{2}}\int_{\varphi(u)}^{\varphi(v)}\int_{\varphi(u)}^{\varphi(v)}W(x,y)dxdy
\end{equation}
%%%%%%%%%%%%%%%%

\blue{I think the explanation above---on how to generate graphs from graphons---is a bit confusing. Maybe separate the two different ways to generate graphs in two different paragraphs, and explain better the meaning of $\varphi$. I guess you could say that $\varphi: V \to [0,1]$ is a function assigning labels in the unit interval to the nodes of the graph.}

As pointed out in~\cite{lovasz2012large} graphons facilitate the understanding of the spectral behavior of sequences of graphs. This was exploited in~\cite{ruiz2019graphon} to extend the concept of Fourier and harmonic analysis to graphons, translating the convolution between filters and signals by means of matrix products into the use of an integral operator that can be applied on signals whose support is contained in $[0,1]$. Graphs obtained from the same graphon by the same procedure have similar spectral characteristics. Indeed, as proven in~\cite{lovasz2012large}[Theorem 11.53] the eigenvalues of graphs in a sequence that converges to a graphon, converge to the eigenvalues of the graphon itself. It was also shown in~\cite{ruiz2019graphon} that the GFT on the graphs converges to the \textit{graphon Fourier transform} given that the signals considered have some structural property. In particular, for any finite graph $G$ with shift operator $\mathbf{S}$ it is possible to associate a graphon $W_{G}$ given by
\begin{equation}
W_{G}(u,v)=\sum_{i=1}^{N}[\mathbf{S}]_{ij}\chi_{\tau_{i}}(u)\chi_{\tau_{j}}(v)
\end{equation}
where $\chi_{\tau_{i}}(u)$ is the characteristic function of the interval $\tau_{i}$ where $\{\tau_{i}\}_{i}^{N}$ forms a partition of $[0,1]$. Accordingly, if there is a graph signal $\mathbf{x}$ defined on $G$ it is possible to associate to it a graphon signal defined on $[0,1]$ which is given by
\begin{equation}
X_{G}(u)=\sum_{i=1}^{N}[\mathbf{x}]_{i}\chi_{\tau_{i}}(u).
\end{equation}
For $\mathbf{x}$ defined on $G$ the graph Fourier transform is given by $\hat{\mathbf{x}}=\mathbf{U}^{T}\mathbf{x}$, where $\mathbf{S}=\mathbf{U}\mathbf{\Lambda}\mathbf{U}^{T}$.

For every graphon $W$ it is possible to define a Hilbert-Schmidt operator acting on a function $X$ defined in $[0,1]$ as
\begin{equation}
\left(T_{W}X\right)(v)=\int_{0}^{1}W(u,v)X(u)du.
\end{equation}
The operator $T_{W}$ is known as the \textit{graphon shift operator} ($W$-SO)~\cite{ruiz2019graphon}. Being $T_{W}$ compact and bounded, it posses a countable set of eigenvalues $\sigma_{1}\geq\sigma_{2}\geq\cdots$ with $0$ as an accumulation point, and associated eigenfunctions $\varphi_{i}(u)$ such that $\sigma_{i}\in [-1,1]$. Using the functions $\varphi_{i}$ it is possible to perform a spectral decomposition of a graphon signal $X$ as follows
\begin{equation}
X=\sum_{i=1}^{\infty}\hat{X}(\sigma_{j})\varphi_{i}
\end{equation}
where
\begin{equation}
\hat{X}(\sigma_{j})=\int_{0}^{1}X(u)\varphi_{j}(u)du.
\end{equation}
The discrete function $\hat{X}$ is known as the \textit{graphon Fourier transform} of $X$. A graphon signal $X$ is called $\omega$-bandlimited
 
 
 

We take advantage of this taking into account that in a graph neural network the convolution is of spectral type and that the signals processed in each layer represent features of common signals.  

In Fig.~\ref{fig:graphon_nn} a graphon neural network with three layers is depicted. The graphon  $W(x,y)$ used to build the graphs in each layer of the network. The mapping between layers of this \textit{graphon} neural network is given by eqn.~(\ref{eq:Hingraph}) where $\mathbf{S}_{\ell}$ equals the adjacency matrix obtained for each case. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
 \centering\includegraphics[angle=-90,scale=0.58]{./figures/fig2T_v01.pdf}
 \caption{Graphon Neural Network}
 \label{fig:graphon_nn}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







==> sec_graphon_nn_v01.tex <==
%!TEX root = GPoolSGNNs_eusipco2020.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Graphon Neural Networks  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Graphon Signal Processing}
A graphon is a symmetric measurable function $W:[0,1]^2\rightarrow\mathbb{R}$ with $0\leq W(x,y)\leq 1$. It was originally conceived as a graph limit for sequences of dense graphs whose number of nodes grows to infinity~\cite{lovasz2012large}. Graphons have also been used as generative models for random graphs~\cite{avella2018centrality} where the entries of the adjacency matrix are sampled as Bernoulli random variables with probability $\kappa W(x_{i},y_{j})$. The constant $\kappa$ defines the sparsity of the graph and $x_{i},y_{j}\in [0,1]$ are selected at random. 

As pointed out in~\cite{lovasz2012large}, the study of graphons facilitates the understanding of several properties of graph sequences. This has been exploited in~\cite{ruiz2019graphon} to extend the concept of convolution to functions associated with graphons, by translating the convolution operation in \eqref{eq:Hingraph} into the use of an integral operator that can be applied to functions supported in $[0,1]$. In particular, for any finite graph $G$ with $\vert V(G)\vert=N$ and shift operator $\mathbf{S}$, it is possible to associate a graphon $W_{G}$ given by
\begin{equation}
W_{G}(u,v)=\sum_{i,j=1}^{N}[\mathbf{S}]_{ij}\chi_{\tau_{i}}(u)\chi_{\tau_{j}}(v)
\end{equation}
where $\chi_{\tau_{i}}(u)$ is the characteristic function of the interval $\tau_{i}$ where $\{\tau_{i}\}_{i=1}^{N}$ forms a partition of $[0,1]$. Accordingly, if there is a graph signal $\mathbf{x}$ defined on $G$ it is possible to associate to it a graphon signal defined on $[0,1]$ which is given by
\begin{equation}
X_{G}(u)=\sum_{i=1}^{N}[\mathbf{x}]_{i}\chi_{\tau_{i}}(u).
\end{equation}
For every graphon $W$ it is possible to define a Hilbert-Schmidt operator acting on a function $X$ defined in $[0,1]$ as
\begin{equation}
\left(T_{W}X\right)(v)=\int_{0}^{1}W(u,v)X(u)du,
\end{equation}
where $T_{W}$ is known as the \textit{graphon shift operator} ($W$-SO) and $X$ is called a \textit{graphon signal}. With these concepts it is possible to define the notion of convolution between a graphon signal $X$ and a \textit{graphon filter} $H=\sum_{k=0}^{K}h_{k}T_{W}^{k}$ with $K$ coefficients as
\begin{equation}
H\ast X=\sum_{k=0}^{K}h_{k}T_{W}^{k}X.
\end{equation} 
%%--------------------------------------------------------------------------------
%%-----------------------------------Section--------------------------------------
%%--------------------------------------------------------------------------------
\section{Graphon Neural Networks: Pooling}\label{sec:graphon_nn}
%%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
 \centering\includegraphics[angle=-90,scale=0.47]{./figures/fig1T_v01.pdf}
 \caption{Different ways to obtain a graph from a graphon.}
 \label{fig:graphfromgraphon}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
 \centering\includegraphics[angle=-90,scale=0.58]{./figures/fig2T_v01.pdf}
 \caption{Graphon Neural Network with three layers}
 \label{fig:graphon_nn}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In light of the results stated in the previous section, we propose to process information on a GNN using a graphon and carry on the filtering of the data using graphon convolutions and a mapping of the data between layers induced by the natural ordering the domain in graphon signals. To do so we generate the layer graphs of the GNN from a graphon. Finite graphs can be obtained from graphons in multiple ways, among which are using sampling and piece-wise approximations (see Fig.~\ref{fig:graphfromgraphon}). In the first case a graph $G=(V(G),E(G),\alpha)$ with nodes set $V(G)$, edge set $E(G)$ and weight function $\alpha:E(G)\rightarrow\mathbb{R}^{+}$ is obtained assigning to each node in $i\in V(G)$ the number $\rho(i)\in [0,1]$, such that for any two nodes $i,j\in V(G)$ we have $\{i,j\}\in E(G)$ and $\alpha(\{i,j\})=W(\rho(i),\rho(j))$, where $\rho: V(G)\rightarrow [0,1]$ is a mapping that defines the type of approximation that is considered to generate the graphs. In the second case a set of $\vert V(G)\vert-1$ points is selected in $[0,1]$ using $\rho$ and for any two nodes $i,j\in V(G)$ we have that $\{i,j\}\in E(G)$ with
%%%%%%%%%%%%%%%%
\begin{equation} \label{eqn:integration}
\alpha(\{i,j\})=\frac{1}{\left\vert \rho(i)-\rho(j)\right\vert^{2}}\int_{\rho(i)}^{\rho(j)}\int_{\rho(i)}^{\rho(j)}W(x,y)dxdy.
\end{equation}
%%%%%%%%%%%%%%%%
Graphs obtained from the same graphon by the same procedure have similar spectral characteristics. Indeed, as proven in~\cite{lovasz2012large} (Theorem 11.53) the eigenvalues of graphs in a sequence that converges to a graphon, converge to the eigenvalues of the graphon itself. It was also shown in~\cite{ruiz2019graphon} that the GFT on the graphs converges to the \textit{graphon Fourier transform} given that the signals considered have some structural property. We exploit this for the processing of signals on a GNN illustrating this concept in Fig.~(\ref{fig:graphon_nn}) where a GNN with three layers is built from a graphon. The graphon  $W(x,y)$ is used to generate the graphs in each layer of the network obtaining the entries of the adjacency matrix using eqn.~(\ref{eqn:integration}). The mapping between layers of this \textit{graphon} neural network is given by eqn.~(\ref{eq:Hingraph}) where $\mathbf{S}_{\ell}$ equals the adjacency matrix obtained for each case. 

To understand why our approach provides an advantage with respect to other approaches, we rely on the connection between harmonic on graphs and  on graphons. Since $T_{W}$ is compact and bounded, it posses a countable set of eigenvalues $1\geq\sigma_{1}\geq\sigma_{2}\geq\cdots 0$ and $-1\leq\sigma_{-1}\leq\sigma_{-2}\leq\cdots 0$ with $0$ as an accumulation point, and associated eigenfunctions $\varphi_{i}(u)$. Using the functions $\varphi_{i}$ it is possible to perform a spectral decomposition of a graphon signal $X$ as follows
\begin{equation}
X=\sum_{i=1}^{\infty}\left(\hat{X}(\sigma_{i})\varphi_{i}+\hat{X}(\sigma_{-i})\varphi_{-i}\right)
\end{equation}
where
\begin{equation}
\hat{X}(\sigma_{j})=\int_{0}^{1}X(u)\varphi_{j}(u)du.
\end{equation}
The discrete function $\hat{X}$ is known as the \textit{graphon Fourier transform} ($W$-FT) of $X$ and a graphon signal $X$ is called $\omega$-bandlimited if there exists $\omega\in (0,1)$ such that $\hat{X}(\sigma_{j})=0$ for all $\vert\sigma_{j}\vert<\omega$.

We recall that for $\mathbf{x}$ defined on $G$ the graph Fourier transform (GFT) is given by $\hat{\mathbf{x}}=\mathbf{U}^{T}\mathbf{x}$, where the GSP has the spectral representation $\mathbf{S}=\mathbf{U}\mathbf{\Lambda}\mathbf{U}^{T}$ with $N$ eigenvalues $\sigma_{1}\geq\sigma_{2}\geq\cdots 0$ and $\sigma_{-1}\leq\sigma_{-2}\leq\cdots 0$. The component of $\hat{\mathbf{x}}$ associated to $\sigma_{j}$ is represented as $\hat{\mathbf{x}}(\sigma_{j})$ and the connection between the $W$-FT and the GFT is given by the following theorem.
\begin{theorem}(\cite{ruiz2019graphon})\label{theorem:graphFTconv}
Let $\{(G_{n},\mathbf{x}_{n})\}$ be a sequence of graph signals converging to the $\omega-$bandlimited graphon signal $(W,X)$, where $T_{W}$ does not have repeated eigenvalues. Then, there exists a sequence of permutations $\pi_{n}$ such that GFT$(\pi_{n}(G_{n}),\pi_{n}(\mathbf{x}))\rightarrow$WFT$(W,X)$ in the sense that $[\hat{\mathbf{x}}]_{j}/\sqrt{n}\rightarrow\hat{X}(\sigma_{j})$ as $n\rightarrow\infty$.
\end{theorem}
One implication of theorem~\ref{theorem:graphFTconv} is the fact that if the signals considered in each layer are equivalent on their spectrum, i.e. they are all bandlimited with the same bandwidth, the filtering on each graph obtained from the graphon is equivalent. These attribute is something shared with the approach proposed in~\cite{gama18-gnnarchit} but with the advantage that there is not ambiguity when mapping signals from one layer to the other. 









==> sec_graphons.tex <==
%!TEX root = GPoolSGNNs_eusipco2020.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
 \centering\includegraphics[angle=-90,scale=0.55]{./figures/fig1T_v00.pdf}
 \caption{Different ways to obtain a graph from a underlying graphon.}
 \label{fig:graphfromgraphon}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A graphon is a symmetric measurable function $W:[0,1]^2\rightarrow\mathbb{R}$ with $0\leq W(x,y)\leq 1$. It was originally conceived as a graph limit for sequences of dense graphs whose number of nodes grows to infinity~\cite{lovasz2012large}. Finite graphs can be obtained from graphons in multiple ways among which are using sampling and step function representations (see Fig.~\ref{fig:graphfromgraphon}). In the first case a graph $G=(V(G),E(G),\alpha)$ with nodes set $V(G)$, edge set $E(G)$ and weight function $\alpha:E(G)\rightarrow\mathbb{R}^{+}$ is obtained selecting a number of $\vert V(G)\vert$ points on $[0,1]$ such that for any two points $u,v$ selected we have $\{u,v\}\in E(G)$ and $\alpha(\{u,v\})=W(u,v)$. In the second case, a set of $\vert V(G)\vert-1$ points is selected in $[0,1]$ and for any two points $u,v$ we have $\{u,v\}\in E(G)$ and 
\begin{equation}
\alpha(\{u,v\})=\int_{\min\{u,v\}}^{\max\{u,v\}}\int_{\min\{u,v\}}^{\max\{u,v\}}W(x,y)dxdy
\end{equation}

As pointed out in~\cite{lovasz2012large} graphons facilitate the understanding of the spectral behavior of sequences of graphs. This was exploited in~\cite{ruiz2019graphon} to extend the concept of Fourier and harmonic analysis to graphons, translating the convolution between a filers and signals by means for matrix products to the use of an integral operator that can be used to consider signals whose support is contained in $[0,1]$.









